Out-of-Distribution Generalization in Text Classification: Past, Present, and Future

Machine learning (ML) systems in natural language processing (NLP) face significant challenges in generalizing to out-of-distribution (OOD) data, where the test distribution differs from the training data distribution. This poses important questions about the robustness of NLP models and their high accuracy, which may be artificially inflated due to their underlying sensitivity to systematic biases. Despite these challenges, there is a lack of comprehensive surveys on the generalization challenge from an OOD perspective in text classification. Therefore, this paper aims to fill this gap by presenting the first comprehensive review of recent progress, methods, and evaluations on this topic. We furth discuss the challenges involved and potential future research directions. By providing quick access to existing work, we hope this survey will encourage future research in this area.

==> bib.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{1}{c|}{\textbf{OOD Scope}}          & \multicolumn{5}{c}{\textbf{Knowledge Transfer}} \\ \midrule

\multicolumn{1}{l|}{Label-Sharing Transfer}       & \multicolumn{5}{l}{\parbox[c]{13cm}{
{Sentiment Analysis}: \cite{kaushik2019learning,Kaushik2021ExplainingTE,hendrycks2020pretrained,Wang2020IdentifyingSC,wang2021robustness,yang2021exploring,kiela2021dynabench,lu2022rationale}; \\ 
{NLI}: \cite{Williams2018ABC,Wang2018GLUEAM,hendrycks2020pretrained,Varshney2020TowardsIS,dranker2021irm,kiela2021dynabench}; \\
{NER}: \cite{jia2019cross,jia2020multi,liu2021crossner,chen2021data,plank2021cross}

} }.      \\ 

\midrule

\multicolumn{1}{l|}{Label-Different Transfer}      & \multicolumn{5}{l}{\parbox[c]{13cm}{
{NER}: \citet{snell2017prototypical,ghaddar2017winer,vu2020effective,wu2020single,Nguyen2021DOZENCZ,cui2021template,ma2021template,zhou2021melm,lee2021good,das2021container,wang2022miner}; \\ 
{Machine Translation}: \citet{Johnson2017GooglesMN,Zhang2020ImprovingMM,Arivazhagan2019TheMI,Ji2020CrosslingualPB,Liu2021ImprovingZT}.}}      \\ \midrule

\multicolumn{1}{c|}{}  & \multicolumn{5}{c}{\textbf{Flexibility of OOD Expressions}}                        \\ \midrule

\multicolumn{1}{l|}{OOD Detection}      & \multicolumn{5}{l}{\parbox[c]{13cm}{NLU: \citet{hendrycks2017baseline,hendrycks2018deep,zheng2020out,hendrycks2020pretrained,zhou2021contrastive,Shen2021EnhancingTG,fort2021exploring}.}}      \\ \midrule

\multicolumn{1}{l|}{OOD Robustness}      & \multicolumn{5}{l}{\parbox[c]{13cm}{Text Classification: \citet{oren2019distributionally,hendrycks2020pretrained,wang2021identifying,du2021towards,liu2021just,Moradi2021EvaluatingTR,Naplava2021UnderstandingMR,Gui2021TextFlintUM}; \\
Natural Language Generation: \citet{Cheng2019RobustNM,zhang2019bridging,zhou2021distributionally,hewitt2021ensembles};\\
Logic Reasoning: \citet{dong2016language,yu2019reclor,liu2021logiqa,zhong2021ar}; \\ 
Evaluations: \citet{czarnowska2019don,kaushik2019learning,gardner2020evaluating,warstadt2020blimp,hu2020xtreme,lewis2020mlqa,lazaridou2021mind,liu2021challenges,koh2021wilds,chen2022can}.}}      \\
\midrule

\multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}Compositional \\ Generalization\end{tabular}} & \multicolumn{5}{l}{\parbox[c]{13cm}{
NLU: \citet{Lake2018GeneralizationWS,russin2019compositional,li2019compositional,gordon2019permutation,andreas2020good,keysers2020measuring,kim2020cogs,kim2021improving}; \\ 
Semantic Parsing: \cite{iyer2017learning,Lake2018GeneralizationWS,dong2018coarse,Lake2019CompositionalGT,furrer2020compositional,kim2021sequence,gupta2022structurally}; \\ 
{Machine Translation}: \citet{chen2020compositional,li2021compositional,zheng2021disentangled} \\
{QA}: \citet{gu2021beyond,lewis2021question,bogin2021latent}
}}.      \\ \midrule

\multicolumn{1}{c|}{}  & \multicolumn{5}{c}{\textbf{Data Noise and Annotation Artifacts}}        \\ \midrule

\multicolumn{1}{l|}{Data Noise}             & \multicolumn{5}{l}{\parbox[c]{13cm}{
Sentiment Analysis: \citet{ganin2016domain,chen2018multinomial,laparra2020rethinking} \\
Machine Translation: \citet{Belinkov2018SyntheticAN,khayrallah2018impact}; \\ 
NER: \citet{liu2021noisy,huang2021nsrl}.}}      \\ \midrule

\multicolumn{1}{l|}{Annotation Artifacts}         & \multicolumn{5}{l}{\parbox[c]{13cm}{
QA: \citet{cai2017pay,min2019compositional,bartolo2021models,bartolo2021improving,lyu2022extending}; \\
NLI: \citet{poliak2018hypothesis,Naik2018StressTE,zellers-etal-2018-swag,feng2019misleading,McCoy2019RightFT,le2020adversarial,sakaguchi2020winogrande,nie-etal-2020-adversarial,liu-etal-2020-hyponli,gardner2021competency,pezeshkpour2022combining,wu2022generating}; \\ 
Sentiment Analysis: \citet{maudslay2019s,zmigrod2019counterfactual,lu2020gender}; \\
Machine Reading Comprehension: \citet{Kaushik2018HowMR,sugawara2018makes,sugawara2020assessing,bartolo2020beat,lai2021machine}; \\
Machine Translation: \citet{Vanmassenhove2018GettingGR,Stanovsky2019EvaluatingGB,tomalin2021practical,choubey2021improving}; \\
Coreference Resolution: \citet{Rudinger2018GenderBI,zhao2018gender}; \\
Toxicity Detection: \citet{Park2018ReducingGB,Dixon2018MeasuringAM}.

} }      \\ \bottomrule
\end{tabular}
}
\caption{A Roadmap for the Scope of Out-Of-Distribution Generalizations.}
\label{table:scope}
\end{table*}

==> name.tex <==
\section{Introduction}\label{intro}
Deep learning and\wyd{\sout{and} including} pre-training technologies have led to significant advances in NLP\wyd{\cite{devlin2018bert,liu2019roberta,radford2018improving}}. On standard benchmarks of machine reading comprehension (MRC) \cite{Kaushik2018HowMR,sugawara2020assessing}, natural language inference (NLI) \cite{Williams2018ABC}, machine translation (MT) \cite{li2021compositional}, question answering (QA) \cite{bogin2021latent,lewis2021question}\wyd{,} and semantic parsing \cite{keysers2020measuring,kim2020cogs}, the state-of-the-art \wyd{(SOTA)} models have given results that are on par with or better than the human-level performance. \wyd{Despite the success of neural models on lots of standard benchmarks including machine reading comprehension (MRC) \cite{Kaushik2018HowMR,sugawara2020assessing}, natural language inference (NLI) \cite{Williams2018ABC} machine translation (MT) \cite{li2021compositional}, question answering (QA) \cite{bogin2021latent,lewis2021question}\wyd{,} and semantic parsing \cite{keysers2020measuring,kim2020cogs}, the superior performance heavily relies on the in-distribution assumption that the training data and the test data share the same distribution. However, the mis-match between the training data distribution and the test data distribution is ubiquitous in the real world, which remains significant challenges when neural models face the out-of-distribution(OOD) problem where the training data distribution is different from the test data distribution~\cite{vapnik1991principles,kawaguchi2017generalization,veitch2019empirical,jung2022machine}. Particularly, the training data distribution and test data distribution in xxx are naturally mis-matched due to xxx reason. Hence it is important to deal with the OOD generalization challenges to further achieve better generalization performance in the test data in the NLP field. Remove the remained sentences.}However, the current technologies still face significant challenges before being practically useful for open-domain real-world applications. For example, it remains an unsolved problem how to transfer knowledge from rich-resource domains and tasks to low-resource ones, and systems demonstrate fragility when there is a slight change in the input. 

\wyd{Although OOD has drawn much attention both in the CV and Time Series fields, it lacks discussion in the NLP field. In this survey, we aim to review existing research in NLP concerning the OOD generalization problem, with the goal of raising awareness of the prevalence of the challenge, and drawing underlying correlations between different lines of works which were previously under noticed.}
Despite difference in the source of challenges above, most of them can be considered as instances of out-of-distribution (OOD) generalization challenges \cite{yang2021generalized}, which are challenges that machine learning models face when the test data distribution differs from the training data. Such challenges are significant to the current deep learning models since most existing research assume that the test data follows the same distribution as the training data, including much research in machine learning on generalization \cite{wang2021generalizing}. Recently, OOD generalization has received increasing attention in the fields of computer vision \cite{koh2021wilds} and Time Series Tasks \cite{gagnon2022woods}. However, relatively little work has discussed OOD generalization formally in NLP, including work that aims to address the aforementioned  problems. 

In this survey, we aim to review existing research in NLP concerning the OOD generalization problem, with the goal of raising awareness of the prevalence of the challenge, and drawing underlying correlations between different lines of works which were previously under noticed. In particular, we identify three main categories of problems in NLP that belong to OOD challenges. The first is cross-domain and cross-task transfer learning tasks, which address systematic distributional variations between training data and test data \cite{hendrycks2020pretrained}. The second is more model-centric, addressing variations between surface text distributions between training and testing data, where there is a true underlying causal distribution that differs from the surface distributions. The third considers unexpected noise or incorrect bias from training data, which can negatively affect the model behavior on test data.

Different methods have been taken to address above issues, which we summarize according to the nature of algorithms. In particular, three main categories of methods have been considered, including data augmentation, invariant feature learning and tailored training strategies. The first category alleviates distributional variances by generating data that bridge the training and test scenarios. Taking the robustness for instance, counterfactuals \cite{Kaushik2021ExplainingTE,Wang2020IdentifyingSC,yang2021exploring,wang2021robustness} have been used to solve spurious pattern issues \cite{kaushik2019learning}. The second category aims to teach model learn features that carry knowledge across different distributions. They are typically used when the test distribution is known \cite{oren2019distributionally}, or can be roughly estimated \cite{vu2020effective,Ji2020CrosslingualPB}. The third category designs dedicated training objective functions or methods to minimize the negative influence of distributional variations \cite{blitzer2006domain,peyrard2021invariant,dranker2021irm}.

Despite the difference in solutions, they all introduce external information for better fitting potential probability distributions. 

[YOU SHOULD DO A CAREFUL READING OF OOD GENERALIZATION SURVEYS IN THE OTHER DOMAINS SO THAT YOU CAN SHOW WHAT HAS BEEN CONSIDERED IN NLP AND WHAT HAS NOT- To be added by Dr Jindong Wang and Yidong]. 

We believe that the survey can provide insight into promising further research directions to solve the OOD generalization problem, thereby advancing NLP towards robust use in the open domain.

% add example draft
\syx{
Examples need to reorganize.

In this survey, NLP OOD generalization problems are summarized in three scopes, Systematic Variance, Training Data Noise and Annotation Artifacts, and Flexibility of Expression, shown in Fig.~\ref{fig:scope}.

Systematic Variance is referring to the variation of the input distribution or the output distribution. One example of variation in input distribution could be the following. For sentiment classification tasks, if the input dataset for training is IMDB movie reviews, while the input dataset for testing is Kindle Book reviews, then the input distribution is variated in terms of tone, word choice, topics, language styles, etc. An example of variation in output distribution could be different label distribution in training and testing name entity recognition datasets. The biomedical training datasets may contain name entity recognition labels relating to CHEMICALs and SYMPTOMs but never cover PERSONs and LOCATIONs labels which is in the testing dataset relating to the news.

Training Data Noise and Annotation Artifacts refer to the flaws and the biased distribution of training datasets. There may be some typos, grammar mistakes, or unknown tokens in the training dataset which may cause the performance degradation of the machine learning models. The training dataset, such as the movie reviews dataset may also be biased and distributed in a way that the comments containing the word “Spielberg” are always under the positive reviews. This may cause the model to learn a shortcut that always makes a positive prediction whenever see the word. 

The boundary between “Training data noise and artifacts” and “flexibility of expression” can be subtle. These two could be distinguished by judging whether the variation exists within the dataset (Training Data Noise and Annotation Artifacts) or is the knowledge learned by the model (Flexibility of Expressions ).

Another scope of OOD generalization problems is the Flexibility of Expression, which study the gap between the pattern that a machine learning model is expected to learn and the feature that the model actually learns due to the statistical distribution of the dataset. One example is the compositional generation of machine translation. A machine translation model can correctly 
translate "Taylor keeps his promise" to Chinese and "James breaks his promise" to Chinese, while it translates "Taylor breaks his promise" incorrectly. In this situation, the model only learn the statistical associate the word “James” with the sentence “breaks his promise”, instead of the ability of understanding and produce the combination of known components.
}
